vMF-Contact: Uncertainty-aware Evidential Learning for Probabilistic Contact-grasp in Noisy Clutter

Grasp learning in noisy environments, such as occlusions, sensor noise, and out-of-distribution (OOD) objects, poses significant challenges. Recent learning-based approaches focus primarily on capturing aleatoric uncertainty from inherent data noise. The epistemic uncertainty, which represents the OOD recognition, is often addressed by ensembles with multiple forward paths, limiting real-time application. In this paper, we propose an uncertainty-aware approach for 6-DoF grasp detection using evidential learning to comprehensively capture both uncertainties in real-world robotic grasping. As a key contribution, we introduce vMF-Contact, a novel architecture for learning hierarchical contact grasp representations with probabilistic modeling of directional uncertainty as von Mises-Fisher (vMF) distribution. To achieve this, we analyze the theoretical formulation of the second-order objective on the posterior parametrization, providing formal guarantees for the model's ability to quantify uncertainty and improve grasp prediction performance. Moreover, we enhance feature expressiveness by applying partial point reconstructions as an auxiliary task, improving the comprehension of uncertainty quantification as well as the generalization to unseen objects. In the real-world experiments, our method demonstrates a significant improvement by 39% in the overall clearance rate compared to the baselines. The code is available under: https://github.com/YitianShi/vMF-Contact/

==> name.tex <==
import os, sys
import pandas as pd
import seaborn as sns
from matplotlib import pyplot
import matplotlib.pyplot as plt
import numpy as np
import argparse
from datetime import datetime
import time, glob, csv
import pandas as pd

# time
current_time = time.time()
# set sns style
sns.set(style="darkgrid", font_scale=1.5)


# helpers
def smooth(scalars, weight):  # Weight between 0 and 1
    last = scalars[0]  # First value in the plot (first timestep)
    smoothed = list()
    for point in scalars:
        smoothed_val = last * weight + (1 - weight) * point  # Calculate smoothed value
        smoothed.append(smoothed_val)                        # Save it
        last = smoothed_val                                  # Anchor the last smoothed value

    return smoothed

def create_lineplot(df, a4_dims, current_time, tag = None, abl=False):
    temp_ = df
    print (temp_.head())
    fig, ax = pyplot.subplots(figsize=a4_dims)
    sns.lineplot(data=temp_, x="Step", y="Success Rate", hue="Method" if not abl else "Online training steps") # turn this into error_bar="se", standardeviation of the mean estimator
    
    plt.legend(loc='best').set_draggable(True)
    

    xscale = np.max(np.asarray(temp_['Step'])) > 5e3
    if xscale:
        # Just some formatting niceness: x-axis scale in scientific notation if max x is large
        plt.ticklabel_format(style='sci', axis='x', scilimits=(0,0))
    plt.tight_layout(pad=0.5)
    str_time = datetime.utcfromtimestamp(current_time).strftime('%Y-%m-%d_%H:%M:%S')
    fig.savefig(f"{tag}.png")
    
def create_barplot(df, a4_dims, current_time, tag = None, bottom = 0.35, abl = False):
    temp_ = df
    print (temp_.head())
    fig, ax = pyplot.subplots(figsize=a4_dims)
    splot = sns.barplot(data=temp_, x="Method" if not abl else "Online training steps", 
                        y="Success Rate", width=.5
                        #, errorbar=("pi", 30)
                        , capsize=.2
                        , ci=None if abl else "deprecated"
                        ) # turn this into error_bar="se", standardeviation of the mean estimator
    axes = splot.axes
    axes.set_ylim(bottom, 1.0)
   
    for g in splot.patches:
        splot.annotate(format(g.get_height()*100, '.1f')+"%",
                    (g.get_x() + g.get_width() / 2., (g.get_height() + bottom) / 2.),
                    ha = 'center', va = 'bottom',
                    xytext = (0, 9),
                    textcoords = 'offset points')
        
    plt.legend(loc='best').set_draggable(True)

    xscale = np.max(np.asarray(temp_['Step'])) > 5e3
    if xscale:
        # Just some formatting niceness: x-axis scale in scientific notation if max x is large
        plt.ticklabel_format(style='sci', axis='x', scilimits=(0,0))
    plt.tight_layout(pad=0.5)
    str_time = datetime.utcfromtimestamp(current_time).strftime('%Y-%m-%d_%H:%M:%S')
    if abl:
        sns.lineplot(data = temp_, marker='o',x="Method" if not abl else "Online training steps", y="Success Rate")
    fig.savefig(f"{tag}.png")

def parse_args():
    parser = argparse.ArgumentParser()
    parser.add_argument('--width', default=11.7, type=float)
    parser.add_argument('--height', default=10, type=float)
    args = parser.parse_args()
    return args

def main(qua, abl = False, group=False):

    args = parse_args()
    a4_dims = (args.width, args.height)


    step_list = []
    success_rate_list = []
    episode_list = []
    method_list = []

    path = "experiments.xls"
    df = pd.ExcelFile(path)
    METHOD_LIST = df.sheet_names
    Quantile_LIST =[a for a in METHOD_LIST if "quan" in a]
    MV_LIST =[a for a in METHOD_LIST if not "quan" in a]
    METHOD_LIST = Quantile_LIST if qua else MV_LIST
    if group:
        abl = False
        METHOD_LIST = ["offline", "online", "online ucb epi ada", "online ucb epi"]
        tags = "epi_"
        if qua:
            METHOD_LIST = [a+" quantile" for a in METHOD_LIST]
            tags = "epi_quantile_"
    else:
        if not qua:
            tags = "epi_ada_" if abl else "MV_" 
        else:
            
            tags = "epi_quantile_ada_" if abl else "QR_"

    for using_method in METHOD_LIST:
        if using_method =='total':
            continue
        elif not group and 'ada' in using_method:
            continue
        
        try:
            int(using_method[0])
            if not abl:
                continue
        except:
            if abl:
                continue
        
                
        
        success_rate_method_list = pd.read_excel(path, using_method, header=None).T.astype('float32').values.tolist()
        
        # using_method += " steps" if abl else ""
        for episode_index, success_rate_episode in enumerate(success_rate_method_list):
            for step_index, success_rate in enumerate(success_rate_episode):
                step_list.append(step_index + 1)
                success_rate_list.append(success_rate)
                episode_list.append(episode_index)
                method_list.append(using_method[:-8] if qua else using_method)

    temp_df = pd.DataFrame(list(zip(step_list, success_rate_list, episode_list, method_list)), \
                                    columns=['Step', 'Success Rate', "Episode", "Method" if not abl else "Online training steps"])
    final = temp_df[temp_df['Step'] == 24]

    print (temp_df.head())
    
    temp_df = temp_df.sort_values(by ='Method' if not abl else "Online training steps").sort_index()
    final = final.sort_values(by ='Method' if not abl else "Online training steps").sort_index()
    create_lineplot(temp_df, a4_dims, current_time, f"{tags}line" , abl=abl)
    create_barplot(final, a4_dims, current_time, f"{tags}bar",abl=abl)
    plt.clf()

if __name__ == '__main__':
    main(abl=True, qua=False)
    main(abl=True, qua=True)
    main(abl=False, qua=True)
    main(abl=False, qua=False)
    main(group=True, qua=False)
    main(group=True, qua=True)


    

